Scalable Semidefinite Relaxation for Maximum A Posterior Estimation

Maximum a posteriori (MAP) inference over discrete Markov random fields is a fundamental task spanning a wide spectrum of real-world applications, which is known to be NP-hard for general graphs. In this paper, we propose a novel semidefinite relaxation formulation (referred to as SDR) to estimate the MAP assignment. Algorithmically, we develop an accelerated variant of the alternating direction method of multipliers (referred to as SDPAD-LR) that can effectively exploit the special structure of the new relaxation. Encouragingly, the proposed procedure allows solving SDR for large-scale problems, e.g., problems on a grid graph comprising hundreds of thousands of variables with multiple states per node. Compared with prior SDP solvers, SDPAD-LR is capable of attaining comparable accuracy while exhibiting remarkably improved scalability, in contrast to the commonly held belief that semidefinite relaxation can only been applied on small-scale MRF problems. We have evaluated the performance of SDR on various benchmark datasets including OPENGM2 and PIC in terms of both the quality of the solutions and computation time. Experimental results demonstrate that for a broad class of problems, SDPAD-LR outperforms state-of-the-art algorithms in producing better MAP assignment in an efficient manner.

==> sdp_section_analysis.tex <==
\section{Theoretical Guarantees: A Family of Optimality Conditions}
\label{Sec:Analysis}

We have derived herein a general set of sufficient conditions for exact MAP inference, which rely only on the potential functions. These optimality conditions are obtained by analyzing the Karush-Kuhn-Kucker conditions for SDPR. As the expressions of these conditions are less informative, we defer them into the Appendix, and present here two samples of applications scenarios for which the proposed condition implies perfect estimation: (i) Image labeling problem~\cite{Hoiem:2007:RSL}, where potential functions are provided by trained classifiers, and (ii) joint image/shape matching from noisy pair-wise matches~\cite{crandall2011discrete}. The proofs are detailed in the supplemental materials.

\subsection{Object Labeling}

In the first example, we consider the image labeling problem as described in~\cite{Hoiem:2007:RSL}, which MAP inference formulation is presented as follows. We have $n$ superpixels of an image, which forms the set of variables. Each superpixel has $m$ potential labels, which represents its states. Let $\set{G}$ connect pairs of super-pixels that are close to each other. Suppose we are given a first-order classifier that provides the first-order potentials $\bs{w}_i$ as well as a second-order classifier that determines the second-order potentials. For simplicity, we assume that the classifiers generate hard outputs, i.e., each element of $\bs{w}_i$ and $\bs{W}_{ij}$ has exactly one non-zero entry being $1$, representing the most probable state or pairs of states predicted by the classifiers, respectively.

Without loss of generality, we assume the optimal states of all super-pixels are the first state, i.e., the underlying group truth to the MAP inference problem is given by $\bs{x}^{gt} = \bs{1}\otimes \bs{e}_1$. The following theorem provides an exact recovery condition on $\bs{w}_i$ and $\bs{W}_{ij}$ under which the SDPR succeeds in recovering $\bs{x}^{gt}$.

\begin{thm} Let the graphs $\set{G}_{\textup{true}}(\set{G}_{\textup{false}})$ encode the set of edges corresponding to the pairwise potentials with correct (incorrect) classification results. Define a vector $\bs{d} = (\bs{d}_1^{T}, \cdots, \bs{d}_{n}^{T})^{T} \in \R^{nm}$ such that
$$
\bs{d}_i = -\bs{w}_i + \sum\nolimits_{(i,j)\in \set{G}_{\textup{false}}} \bs{W}_{ij}\bs{1}.
$$
Then $\bs{x}^{gt} = \bs{1}\otimes \bs{e}_1$ is the unique global optimal of SDPR if
\begin{equation}
\lambda_{2}(\set{G}_{\textup{true}}) > 2\|\bs{d}\|_{\infty},
\label{Eq:Label}
\end{equation}
where $\lambda_{2}(\set{G}_{\textup{true}})$ is the algebraic connectivity of $\set{G}_{\textup{true}}$.
\end{thm}

An interesting fact about~(\ref{Eq:Label}) is that $\|\bs{d}\|_{\infty}$ is a measure on the magnitude of the structure of the noisy measurement. This arises since the sum of magnitudes of all elements in $\bs{d}$ is bounded by $O(|\set{E}_{\textup{false}}|)$. Thus when each noisy measurement is randomly drawn, then energy of $\bs{d}$ is uniformly distributed across all elements. In this case, the expected value of $\|\bs{d}\|_{\infty}$ is only $O(|\set{E}_{\textup{false}}|/(nm))$. In other words, if the noise energy is reasonably spread out, then we can tolerate the highest level of noise.

\subsection{Joint Shape Matching}

As a second example, we consider the problem of matching multiple rigid objects from pair-wise transformation measurements, which is a fundamental problem across many field such as structure from motion~\cite{crandall2011discrete} and organizing of a collection of shapes~\cite{hsg-fgssl-13}. In this setting, we are given $n$ shapes $\set{S}_1,\cdots, \set{S}_{n}$ and a set of noisy relative transformations estimated between pairs of shapes specified by a graph $\set{G}$. The goal is to find the transformation of each shape with respect to a fixed shape (say $\set{S}_1$), such that the induced relative transformations agree with the input relative transformations as much as possible. So far, the best known theoretical guarantee on joint shape matching is that in a randomized setting, one can recover the ground-truth transformations if the amount of noise, i.e., the percentage of incorrect pair-wise relative transformations is below $50\%$~\cite{Wang:2013:FSA}. In~\cite{crandall2011discrete}, the authors provide a MRF formulation for the joint shape matching problem. We show that this formulation allows us to substantially improve the noise tolerance level.

Without loss of generality, we consider the simplified setting of matching 1D rotations, e.g., matching the orientations of 3D shapes around the $z$ axis. In this case, we assume each shape is given $m$ candidate orientations (i.e., they describe the states of each shape), uniformly distributed between $0^{\circ}$ and $360^{\circ}$, i.e., $360^{\circ}*k/m, 0\leq k \leq m-1$. Each input relative transformation gives a measurement on the absolute difference between the orientations of the two shapes. Thus, the potential functions admit the forms
$$\footnotesize
\bs{w}_i = \left\{
                    \begin{array}{cc}
                     \bs{e}_{i_{k}} & (1,i) \in \set{G},\\
                     0 & \textup{otherwise},\\
                    \end{array}
                  \right.\, \ \bs{W}_{ij} = \left\{
                    \begin{array}{cc}
                     \bs{Q}_{k(i,j)} & (i,j) \in \set{G},\\
                     0 & \textup{otherwise},\\
                    \end{array}
                  \right.\,
$$
where $\bs{Q}_{k(i,j)}$ is given by the identity matrix or one of the $m-1$ permutations that slide the row (or columns) of $I_{n}$ by a constant number. For example, in the case of $m=3$
$$
\footnotesize
\quad \bs{Q}_1 = \left(
             \begin{array}{ccc}
               0 & 1 & 0 \\
               0 & 0 & 1 \\
               1 & 0 & 0 \\
             \end{array}
           \right),\quad \bs{Q}_2 = \left(
             \begin{array}{ccc}
               0 & 0 & 1 \\
               1 & 0 & 0 \\
               0 & 1 & 0 \\
             \end{array}
           \right).
$$
The goal is to label each shape as one of the orientation.

To get a more informative understanding of the exact recovery condition of SDPR in this section, we present a randomized setting, where independently (i) $\set{G}$ follows the Erdos-Renyi random graph model with edge selection probability $p_{\textup{obs}}$, (ii) The wrong pair-wise measurement has probability $p_{\textup{false}}$, and (iii) the wrong pair-wise measurements are uniformly distributed within $360^{\circ}*k/m, 1\leq k \leq m-1$.

\begin{thm} Consider the above randomized model. For any small constant $\delta > 0$, there exists a numerical constant $c>0$ such that SDPR admits exact recovery with probability at least $1 - \frac{2}{(nm)^{10}}$, provided that
\begin{equation}
p_{\textup{false}} < \frac{1-\delta}{1+\delta}\frac{2}{3-1/m},
\label{Bound:Opt}
\end{equation}
and
$$
p_{\textup{false}}p_{\textup{obs}}/m > c\log(mn)/n
$$
\end{thm}

Theorem \ref{Bound:Opt} asserts that the noise tolerance level converges rapidly to $66\%$ with high probability, which improves upon the best-known result ~\cite{Wang:2013:FSA}. One way to understand this is that, similar to the first example, when the corrupted relative transformation measurements are uniformly distributed, they tend to not agree with each other, or in other words, there do not exist strong sub-graphs among the wrong pairs. This explains why we can tolerate more than $50\%$ noise. Note that the ability to capture the structure of the noise is enabled by our MAP formulation, which utilizes a discrete set of candidate orientations of each shape. The alternative approach of~\cite{crandall2011discrete}, which directly optimizes the transformation of each shape through convex optimization, can only obtain bounds on the amount of noise.

Note that unlike the first example, where we obtain a noise bound on the order of $1-O(1/m)$, in this application setting we are only able to obtain a constant bound. This can be understood by the difference between the measurements in both settings, namely, in the first example, the pair-wise potential indicates both the states of variables, while the in the second setting, the measurement only indicates the relative optimal states --- a much weaker constraint.

